Robustness Meets Deep Learning: An End-to-End Hybrid Pipeline for Unsupervised Learning of Egomotion

In this work, we propose a method that combines unsupervised deep learning predictions for optical flow and monocular disparity with a model based optimization procedure for instantaneous camera pose. Given the flow and disparity predictions from the network, we apply a RANSAC outlier rejection scheme to find an inlier set of flows and disparities, which we use to solve for the relative camera pose in a least squares fashion. We show that this pipeline is fully differentiable, allowing us to combine the pose with the network outputs as an additional unsupervised training loss to further refine the predicted flows and disparities. This method not only allows us to directly regress relative pose from the network outputs, but also automatically segments away pixels that do not fit the rigid scene assumptions that many unsupervised structure from motion methods apply, such as on independently moving objects. We evaluate our method on the KITTI dataset, and demonstrate state of the art results, even in the presence of challenging independently moving objects.

==> tex/ablation_losses.tex <==
\begin{figure}
\centering
    \includegraphics[width=.45\linewidth]{images/disp-bf-rfine.png}
    \includegraphics[width=.45\linewidth]{images/flow-bf-rfine.png}
    \includegraphics[width=.45\linewidth]{images/disp-in-rfine.png}
    \includegraphics[width=.45\linewidth]{images/flow-in-rfine.png}
    \includegraphics[width=.45\linewidth]{images/rsc-disp-loss.png}
    \includegraphics[width=.45\linewidth]{images/rsc-flow-loss.png}
\includegraphics[width=.45\linewidth]{images/inlier.png}
\caption{Plots of training losses against number of training iterations. Left column is for the disparity losses and right column is for the flow. The first row shows the the losses before the refinement, and the last two rows shows the original losses and the refinement losses after the refinement losses are added.}
\label{fig:refine-loss}
\end{figure}

==> tex/discussion.tex <==
\section{Discussion}
\label{sec:discussion}
\TODO{Update}
From our experiments, we can see that our pose prediction results are competitive with most state of the art methods. Overall, DVSO clearly beats the other methods, but relies on a joint optimization scheme that allows for optimization over multiple long term keyframes. On the other hand, our method's pose predictions are generated by concatenating pose estimates between each pair of frames in each sequence, and so could see significant improvement with a similar optimization scheme. Amongst the other methods, we outperform the monocular only SFMLearner and the work by Zhan et al., are quite close to UnDeepVO, but do not achieve the same accuracy as Luo et al. However, this work takes as input images of size 256x832, and so receive a significantly larger amount of information to process. 

In our ablations, we saw that our pose results improve significantly given the additional refinement, but we did not see a similar improvement in the flow and depth errors. To resolve these two conflicting sets of results, we additionally computed the flow and depth error metrics only over points considered inliers by RANSAC, which we show in Tables \ref{tab:inlier_only_flow} and \ref{tab:inlier_only_depth}. From these results, we can see that our inlier flow errors improve significantly after refinement, with a more modest improvement in the depth errors. This follows from the formulation of our loss, as it only allows for backpropagation through the inlier points. However, while the errors over these inlier points have improved, the outlier points experienced worse errors, resulting in a lower than expected improvement in global errors. This is not an issue when the goal is pose estimation, and only the inliers are used to estimate pose, but in the future, we plan to explore better ways to combine these losses to improve the global errors further.

==> tex/table.tex <==
\begin{table*}[t!]
\centering
 \begin{tabular}{ccccccccc} 
 \hline\\[-1ex]
  \textbf{outdoor$\_$day2} & \multicolumn{4}{c}{Average Depth Error (m)} & \multicolumn{4}{c}{Average Height Error (m)}\\
  Depth Threshold & 5m & 10m & 20m & 100m & 5m & 10m & 20m & 100m \\ [0.5ex]
 \hline \\[-1ex]
 ipm-raw-depth5 &  30.52 & 29.88 & 28.46 & 25.87 & 3.13 & 3.43 & 3.57 & 3.34 \\
ipm-raw-image1 &  2.92 & 5.54 & 9.29 & 16.28 & 0.9 & 1.23 & 1.64 & 2.12 \\
ipm-raw-fixed-plane4 &  7.42 & 10.72 & 14.25 & 16.43 & 1.85 & 2.31 & 2.8 & 2.91 \\
 \hline\\[-1ex]
  \textbf{outdoor$\_$day1} & \multicolumn{4}{c}{Average Depth Error (m)} & \multicolumn{4}{c}{Average Height Error (m)}\\
  Depth Threshold & 5m & 10m & 20m & 100m & 5m & 10m & 20m & 100m \\ [0.5ex]
 \hline \\[-1ex]
 ipm-raw-depth5 &  25.91 & 26.78 & 26.74 & 24.9 & 2.87 & 3.28 & 3.94 & 4.27 \\
ipm-raw-image1 &  3.83 & 5.73 & 9.89 & 16.86 & 0.93 & 1.42 & 2.19 & 2.95 \\
ipm-raw-fixed-plane4 &  6.75 & 8.7 & 12.5 & 16.36 & 1.66 & 2.29 & 3.17 & 3.79 \\
 \hline\\[-1ex]
  \textbf{outdoor$\_$night3} & \multicolumn{4}{c}{Average Depth Error (m)} & \multicolumn{4}{c}{Average Height Error (m)}\\
  Depth Threshold & 5m & 10m & 20m & 100m & 5m & 10m & 20m & 100m \\ [0.5ex]
 \hline \\[-1ex]
 ipm-raw-depth5 &  25.82 & 27.42 & 26.81 & 24.91 & 3.92 & 4.1 & 4.32 & 3.91 \\
ipm-raw-image1 &  4.38 & 5.96 & 10.06 & 14.27 & 1.23 & 1.61 & 2.25 & 2.56 \\
ipm-raw-fixed-plane4 &  5.95 & 8.49 & 12.52 & 14.54 & 1.69 & 2.41 & 3.16 & 3.24
\end{tabular}
\caption{}
\label{tab:depth_height_results}
\end{table*}
